A network-based transfer learning approach to improve sales forecasting of new products

Data-driven methods -- such as machine learning and time series forecasting -- are widely used for sales forecasting in the food retail domain. However, for newly introduced products insufficient training data is available to train accurate models. In this case, human expert systems are implemented to improve prediction performance. Human experts rely on their implicit and explicit domain knowledge and transfer knowledge about historical sales of similar products to forecast new product sales. By applying the concept of Transfer Learning, we propose an analytical approach to transfer knowledge between listed stock products and new products. A network-based Transfer Learning approach for deep neural networks is designed to investigate the efficiency of Transfer Learning in the domain of food sales forecasting. Furthermore, we examine how knowledge can be shared across different products and how to identify the products most suitable for transfer. To test the proposed approach, we conduct a comprehensive case study for a newly introduced product, based on data of an Austrian food retailing company. The experimental results show, that the prediction accuracy of deep neural networks for food sales forecasting can be effectively increased using the proposed approach.

==> table_results_all.tex <==
\begin{tabular}
  {@{} 
    lccccccccccccccc|cccc
  @{}}
  \toprule
    & \multicolumn{15}{c}{Validation weeks} &
      \multicolumn{4}{c}{Average results} & \\
    &  \multicolumn{1}{c} {W3} & {W4} & {W5} & \underline{{W6}}& \underline{{W7}}& \underline{{W8}}& \underline{{W9}}& \underline{{W10}}& {W11}& \underline{{W12}}& {W13}& {W14}& {W15}& {W16}& {W17}& {Weeks w/o promo}& \underline{{Weeks w/ promo}}& {Weeks total} & {Improvement}\\
  \midrule
w/o Transfer &   6.26  \num{+-1.06} &   5.16  \num{+-0.58} &   4.7  \num{+-0.2} &   29.12  \num{+-12.06} &   27.67  \num{+-8.5} &   20.92  \num{+-0.44} &   28.04  \num{+-0.46} &   21.65  \num{+-1.19} &   10.8  \num{+-4.13} &   24.69  \num{+-1.69} &   5.53  \num{+-0.3} &   4.87  \num{+-0.27} &   4.98  \num{+-0.11} &   4.68  \num{+-0.1} &   3.95  \num{+-0.18} &   5.66  \num{+-0.77} &   25.35  \num{+-4.06} &   13.53  \num{+-2.08} &    \\
Naive & 5.80 & 5.28 & 5.05 & 14.71 & 16.90 & 23.03 & 31.20 & 21.79 & 9.79 & 26.72 & 7.65 & 6.97 & 6.37 & 6.41 & 5.65 & 6.55 & 22.39 & 12.89 & \\
 \bottomrule
 Config. 1 \\
Source 1 &   12.17  \num{+-4.37} &   4.67  \num{+-0.09} &   4.6  \num{+-0.04} &   81.26  \num{+-143.61} &   18.74  \num{+-5.71} &   21.54  \num{+-0.4} &   27.9  \num{+-0.28} &   25.62  \num{+-2.31} &   6.91  \num{+-0.09} &   29.36  \num{+-1.18} &   6.54  \num{+-0.55} &   4.87  \num{+-0.17} &   5  \num{+-0.08} &   4.65  \num{+-0.05} &   3.93  \num{+-0.06} &   5.93  \num{+-0.61} &   34.07  \num{+-25.58} &   17.18  \num{+-10.6} & 7/15 \\
Source 2 &   22.64  \num{+-6.05} &   5.32  \num{+-0.51} &   5.23  \num{+-0.52} &   15.37  \num{+-2.2} &   15.52  \num{+-0.26} &   21.44  \num{+-0.4} &   27.94  \num{+-0.19} &   24.19  \num{+-1.4} &   6.87  \num{+-0.09} &   25.02  \num{+-1.06} &   6  \num{+-0.39} &   4.76  \num{+-0.09} &   4.96  \num{+-0.06} &   4.65  \num{+-0.05} &   3.92  \num{+-0.05} &   7.15  \num{+-0.87} &   21.58  \num{+-0.92} &   12.92  \num{+-0.89} & 8/15 \\
Source 3 &   5.18  \num{+-0.11} &   4.71  \num{+-0.05} &   4.57  \num{+-0.03} &   13.78  \num{+-0.65} &   17.1  \num{+-1.47} &   21.02  \num{+-0.33} &   27.84  \num{+-0.36} &   21.46  \num{+-0.73} &   7.11  \num{+-0.34} &   24.78  \num{+-0.74} &   5.35  \num{+-0.1} &   4.73  \num{+-0.08} &   4.93  \num{+-0.04} &   \textbf{4.62}  \num{+-0.05} &   3.9  \num{+-0.06} &   5.01  \num{+-0.1} &   21  \num{+-0.71} &   11.41  \num{+-0.34} & 13/15 \\
Source 4 &   5.01  \num{+-0.04} &   4.68  \num{+-0.05} &   4.57  \num{+-0.03} &   14.06  \num{+-0.51} &   14.33  \num{+-0.42} &   34.89  \num{+-6.7} &   27.98  \num{+-0.48} &   21.66  \num{+-0.84} &   6.98  \num{+-0.13} &   24.36  \num{+-0.46} &   5.32  \num{+-0.12} &   4.76  \num{+-0.13} &   4.93  \num{+-0.05} &   4.64  \num{+-0.07} &   3.91  \num{+-0.05} &   \textbf{4.98}  \num{+-0.07} &   22.88  \num{+-1.57} &   12.14  \num{+-0.67} & 13/15 \\
Source 5 &   5.02  \num{+-0.05} &   4.65  \num{+-0.03} &   4.56  \num{+-0.02} &   14.87  \num{+-0.45} &   18.03  \num{+-4.31} &   23.17  \num{+-1.35} &   28.35  \num{+-0.56} &   21.83  \num{+-1.7} &   7.78  \num{+-0.44} &   23.95  \num{+-0.81} &   \textbf{5.3} \num{+-0.09} &   4.72  \num{+-0.1} &   4.94  \num{+-0.03} &   4.63  \num{+-0.04} &   3.92  \num{+-0.08} &   5.06  \num{+-0.1} &   21.7  \num{+-1.53} &   11.71  \num{+-0.67} & 12/15 \\
Source 6 &   5.21  \num{+-0.11} &   4.72  \num{+-0.05} &   4.57  \num{+-0.02} &   13.2  \num{+-0.88} &   16.46  \num{+-1.55} &   \textbf{20.87}  \num{+-0.23} &   27.18  \num{+-0.41} &   21.56  \num{+-0.94} &   \textbf{6.85}  \num{+-0.07} &   24.99  \num{+-0.89} &   5.49  \num{+-0.14} &   4.7  \num{+-0.07} &   4.94  \num{+-0.05} &   4.63  \num{+-0.05} &   3.91  \num{+-0.07} &   5  \num{+-0.07} &   20.71  \num{+-0.82} &   11.29  \num{+-0.37} & \textbf{14/15} \\
Source 7 &   5.04  \num{+-0.07} &   4.76  \num{+-0.07} &   4.56  \num{+-0.02} &   16.4  \num{+-0.76} &   14.07  \num{+-0.49} &   24.41  \num{+-2.82} &   27.26  \num{+-0.43} &   21.83  \num{+-1.18} &   7.06  \num{+-0.11} &   23.82  \num{+-0.79} &   5.37  \num{+-0.08} &   \textbf{4.69}  \num{+-0.04} &   \textbf{4.92}  \num{+-0.04} &   4.63  \num{+-0.03} &   3.9  \num{+-0.05} &   4.99  \num{+-0.06} &   21.3  \num{+-1.08} &   11.51  \num{+-0.46} & 13/15 \\
Source 8 &   4.98  \num{+-0.03} &   4.73  \num{+-0.07} &   4.58  \num{+-0.03} &   15.73  \num{+-0.46} &   14.68  \num{+-0.48} &   26.78  \num{+-4.66} &   27.89  \num{+-0.47} &   21.73  \num{+-0.82} &   7.09  \num{+-0.22} &   24.49  \num{+-0.73} &   5.39  \num{+-0.11} &   4.71  \num{+-0.07} &   4.96  \num{+-0.05} &   \textbf{4.62}  \num{+-0.03} &   \textbf{3.89}  \num{+-0.06} &   5  \num{+-0.08} &   21.88  \num{+-1.27} &   11.75  \num{+-0.55} & 13/15 \\
Source 9 &   5.1  \num{+-0.06} &   4.73  \num{+-0.06} &   4.56  \num{+-0.02} &   15.64  \num{+-0.68} &   16.63  \num{+-2.18} &   23.51  \num{+-2.19} &   27.96  \num{+-0.63} &   21.59  \num{+-1.31} &   7.32  \num{+-0.25} &   25.11  \num{+-0.85} &   5.34  \num{+-0.09} &   4.71  \num{+-0.08} &   4.94  \num{+-0.08} &   4.64  \num{+-0.07} &   3.92  \num{+-0.08} &   5.03  \num{+-0.09} &   21.74  \num{+-1.31} &   11.71  \num{+-0.58} & 13/15 \\
Source 10 &   5.13  \num{+-0.06} &   4.79  \num{+-0.05} &   4.58  \num{+-0.02} &   15.05  \num{+-1.07} &   14.7  \num{+-0.25} &   22.34  \num{+-2.13} &   28.41  \num{+-0.77} &   22.03  \num{+-1.37} &   6.99  \num{+-0.1} &   24.7  \num{+-0.6} &   5.41  \num{+-0.14} &   4.73  \num{+-0.06} &   \textbf{4.92}  \num{+-0.03} &   4.65  \num{+-0.04} &   3.96  \num{+-0.14} &   5.02  \num{+-0.07} &   21.2  \num{+-1.03} &   11.49  \num{+-0.46} & 11/15 \\
Source 11 &   5.33  \num{+-0.12} &   4.76  \num{+-0.06} &   4.58  \num{+-0.02} &   13.32  \num{+-0.49} &   21.31  \num{+-5.91} &   21.32  \num{+-0.8} &   \textbf{26.99}  \num{+-0.38} &   22.05  \num{+-0.99} &   7.13  \num{+-0.21} &   25.55  \num{+-0.77} &   5.35  \num{+-0.11} &   4.71  \num{+-0.07} &   4.93  \num{+-0.04} &   4.63  \num{+-0.04} &   3.91  \num{+-0.07} &   5.04  \num{+-0.08} &   21.75  \num{+-1.56} &   11.72  \num{+-0.67} & 12/15 \\
Source 12 &   5.15  \num{+-0.09} &   4.72  \num{+-0.06} &   4.56  \num{+-0.02} &   15.56  \num{+-0.99} &   15.78  \num{+-0.77} &   21.21  \num{+-0.6} &   27.63  \num{+-0.44} &   21.58  \num{+-1.07} &   6.92  \num{+-0.1} &   24.38  \num{+-0.62} &   5.41  \num{+-0.17} &   4.72  \num{+-0.06} &   4.95  \num{+-0.04} &   4.64  \num{+-0.03} &   3.92  \num{+-0.08} &   5  \num{+-0.07} &   21.02  \num{+-0.75} &   11.41  \num{+-0.34} & \textbf{14/15} \\
Source 13 &   5.24  \num{+-0.06} &   4.77  \num{+-0.06} &   4.56  \num{+-0.02} &   14.39  \num{+-0.48} &   15.59  \num{+-0.58} &   22.11  \num{+-0.76} &   27.65  \num{+-0.37} &   22.25  \num{+-1.43} &   6.94  \num{+-0.11} &   24.23  \num{+-0.46} &   5.39  \num{+-0.16} &   4.71  \num{+-0.07} &   4.94  \num{+-0.05} &   4.66  \num{+-0.07} &   3.91  \num{+-0.06} &   5.01  \num{+-0.07} &   21.04  \num{+-0.68} &   11.42  \num{+-0.32} & 13/15 \\
Source 14 &   5.14  \num{+-0.05} &   4.78  \num{+-0.07} &   4.58  \num{+-0.02} &   14.88  \num{+-0.45} &   14.81  \num{+-0.61} &   21.59  \num{+-0.59} &   27.67  \num{+-0.45} &   21.75  \num{+-0.86} &   7.33  \num{+-0.21} &   23.44  \num{+-0.27} &   5.4  \num{+-0.11} &   4.71  \num{+-0.07} &   4.93  \num{+-0.07} &   4.66  \num{+-0.06} &   3.91  \num{+-0.05} &   5.05  \num{+-0.08} &   20.69  \num{+-0.54} &   11.3  \num{+-0.26} & 13/15 \\

\bottomrule
Config. 2 \\
Source 1 &   9.73  \num{+-3.35} &   4.8  \num{+-0.24} &   4.75  \num{+-0.21} &   20.44  \num{+-11.73} &   17.03  \num{+-1.95} &   21.73  \num{+-0.55} &   28.31  \num{+-0.43} &   26.32  \num{+-2.05} &   7.04  \num{+-0.11} &   33.04  \num{+-1.12} &   10.89  \num{+-3.98} &   4.82  \num{+-0.14} &   5.1  \num{+-0.13} &   4.68  \num{+-0.07} &   4.07  \num{+-0.12} &   6.21  \num{+-0.93} &   24.48  \num{+-2.97} &   13.52  \num{+-1.75} & 6/15 \\
Source 2 &   11.19  \num{+-3.22} &   5  \num{+-0.28} &   4.81  \num{+-0.19} &   15.47  \num{+-4.48} &   15.89  \num{+-0.36} &   22.8  \num{+-0.44} &   28.74  \num{+-0.53} &   24.86  \num{+-1.4} &   7.01  \num{+-0.07} &   26.07  \num{+-0.6} &   7.96  \num{+-1.2} &   4.85  \num{+-0.14} &   5.07  \num{+-0.09} &   4.68  \num{+-0.06} &   4.01  \num{+-0.13} &   6.06  \num{+-0.6} &   22.3  \num{+-1.3} &   12.56  \num{+-0.88} & 6/15 \\
Source 3 &   5.29  \num{+-0.12} &   4.67  \num{+-0.03} &   4.57  \num{+-0.02} &   12.61  \num{+-0.35} &   16.55  \num{+-0.88} &   21.34  \num{+-0.33} &   27.98  \num{+-0.39} &   20.94  \num{+-0.49} &   6.94  \num{+-0.13} &   24.52  \num{+-0.51} &   5.45  \num{+-0.11} &   4.85  \num{+-0.09} &   4.97  \num{+-0.06} &   4.68  \num{+-0.09} &   3.98  \num{+-0.06} &   5.04  \num{+-0.08} &   20.66  \num{+-0.49} &   11.29  \num{+-0.24} & 13/15 \\
Source 4 &   4.98  \num{+-0.03} &   4.7  \num{+-0.06} &   4.57  \num{+-0.01} &   13.71  \num{+-0.32} &   14.29  \num{+-0.21} &   22.25  \num{+-1.11} &   28.32  \num{+-0.38} &   20.69  \num{+-0.28} &   6.92  \num{+-0.06} &   25.53  \num{+-0.64} &   \textbf{5.3} \num{+-0.03} &   4.83  \num{+-0.13} &   4.94  \num{+-0.04} &   4.64  \num{+-0.04} &   3.96  \num{+-0.06} &   \textbf{4.98}  \num{+-0.05} &   20.8  \num{+-0.49} &   11.31  \num{+-0.23} & 12/15 \\
Source 5 &   5.04  \num{+-0.06} &   \textbf{4.63}  \num{+-0.02} &   4.57  \num{+-0.03} &   15.18  \num{+-0.49} &   22.14  \num{+-10.73} &   23.42  \num{+-1.5} &   28.86  \num{+-0.92} &   20.73  \num{+-0.39} &   8.51  \num{+-0.39} &   23.6  \num{+-0.52} &   5.56  \num{+-0.12} &   4.74  \num{+-0.06} &   5.01  \num{+-0.06} &   4.64  \num{+-0.04} &   3.91  \num{+-0.04} &   5.18  \num{+-0.09} &   22.32  \num{+-2.42} &   12.04  \num{+-1.02} & 11/15 \\
Source 6 &   5.33  \num{+-0.11} &   4.69  \num{+-0.04} &   4.59  \num{+-0.03} &   \textbf{12.53}  \num{+-1.12} &   14.63  \num{+-0.44} &   21.32  \num{+-0.16} &   27.9  \num{+-0.5} &   21.6  \num{+-0.83} &   6.91  \num{+-0.07} &   24.23  \num{+-0.31} &   5.66  \num{+-0.14} &   4.72  \num{+-0.06} &   4.95  \num{+-0.03} &   4.67  \num{+-0.07} &   3.97  \num{+-0.07} &   5.06  \num{+-0.07} &   \textbf{20.37}  \num{+-0.56} &   \textbf{11.18}  \num{+-0.27} & 13/15 \\
Source 7 &   5.01  \num{+-0.03} &   4.82  \num{+-0.07} &   4.58  \num{+-0.01} &   16.61  \num{+-0.37} &   \textbf{13.87}  \num{+-0.45} &   22.38  \num{+-0.38} &   28.63  \num{+-0.41} &   21.13  \num{+-0.59} &   7.18  \num{+-0.12} &   23.45  \num{+-0.26} &   5.49  \num{+-0.12} &   4.72  \num{+-0.04} &   4.94  \num{+-0.06} &   4.66  \num{+-0.03} &   3.97  \num{+-0.06} &   5.04  \num{+-0.06} &   21.01  \num{+-0.41} &   11.43  \num{+-0.2} & 13/15 \\
Source 8 &   4.99  \num{+-0.03} &   4.78  \num{+-0.07} &   4.58  \num{+-0.02} &   16.15  \num{+-0.34} &   14.63  \num{+-0.18} &   21.41  \num{+-0.28} &   29.66  \num{+-0.38} &   20.45  \num{+-0.22} &   7.28  \num{+-0.2} &   23.84  \num{+-0.29} &   5.73  \num{+-0.19} &   4.97  \num{+-0.13} &   5.04  \num{+-0.07} &   4.66  \num{+-0.05} &   3.96  \num{+-0.06} &   5.11  \num{+-0.09} &   21.02  \num{+-0.28} &   11.48  \num{+-0.17} & 10/15 \\
Source 9 &   5.05  \num{+-0.04} &   4.74  \num{+-0.06} &   4.58  \num{+-0.02} &   15.17  \num{+-0.42} &   15.15  \num{+-1.87} &   23.19  \num{+-1.27} &   27.83  \num{+-0.34} &   20.68  \num{+-0.39} &   7.15  \num{+-0.15} &   24.47  \num{+-0.23} &   5.44  \num{+-0.11} &   5  \num{+-0.11} &   4.98  \num{+-0.03} &   4.67  \num{+-0.04} &   4.02  \num{+-0.06} &   5.07  \num{+-0.07} &   21.08  \num{+-0.75} &   11.48  \num{+-0.34} & 12/15 \\
Source 10 &   5.15  \num{+-0.05} &   4.74  \num{+-0.05} &   4.61  \num{+-0.01} &   15.17  \num{+-0.68} &   15.07  \num{+-0.27} &   21.65  \num{+-0.51} &   29.25  \num{+-0.5} &   20.93  \num{+-0.63} &   7.14  \num{+-0.14} &   \textbf{23.35}  \num{+-0.46} &   5.55  \num{+-0.14} &   4.78  \num{+-0.05} &   4.95  \num{+-0.02} &   4.69  \num{+-0.04} &   3.99  \num{+-0.05} &   5.07  \num{+-0.06} &   20.9  \num{+-0.51} &   11.4  \num{+-0.24} & 11/15 \\
Source 11 &   5.39  \num{+-0.13} &   4.77  \num{+-0.04} &   4.64  \num{+-0.06} &   12.91  \num{+-0.51} &   16.33  \num{+-1.73} &   21.38  \num{+-0.24} &   27.45  \num{+-0.34} &   22.74  \num{+-0.96} &   7.11  \num{+-0.13} &   24.72  \num{+-0.38} &   5.41  \num{+-0.1} &   4.76  \num{+-0.06} &   4.94  \num{+-0.04} &   4.65  \num{+-0.04} &   3.94  \num{+-0.04} &   5.07  \num{+-0.07} &   20.92  \num{+-0.69} &   11.41  \num{+-0.32} & 12/15 \\
Source 12 &   5.09  \num{+-0.04} &   4.79  \num{+-0.05} &   4.64  \num{+-0.04} &   14.07  \num{+-1.57} &   14.69  \num{+-0.25} &   21.36  \num{+-0.25} &   28.27  \num{+-0.39} &   21.65  \num{+-0.69} &   7.64  \num{+-0.22} &   23.73  \num{+-0.32} &   5.69  \num{+-0.22} &   5.07  \num{+-0.12} &   5.04  \num{+-0.07} &   4.76  \num{+-0.08} &   3.98  \num{+-0.05} &   5.19  \num{+-0.1} &   20.63  \num{+-0.58} &   11.36  \num{+-0.29} & 8/15 \\
Source 13 &   5.27  \num{+-0.07} &   4.76  \num{+-0.05} &   4.59  \num{+-0.02} &   14.24  \num{+-0.3} &   16.39  \num{+-2.3} &   22.83  \num{+-0.73} &   28.89  \num{+-0.49} &   20.13  \num{+-0.16} &   7.17  \num{+-0.12} &   24.26  \num{+-0.3} &   5.48  \num{+-0.12} &   4.82  \num{+-0.08} &   4.97  \num{+-0.04} &   4.7  \num{+-0.05} &   3.99  \num{+-0.08} &   5.08  \num{+-0.07} &   21.12  \num{+-0.71} &   11.5  \num{+-0.33} & 12/15 \\
Source 14 &   5.1  \num{+-0.04} &   4.78  \num{+-0.05} &   4.63  \num{+-0.01} &   14.59  \num{+-0.36} &   14.96  \num{+-0.75} &   21.66  \num{+-0.28} &   28.37  \num{+-0.45} &   20.77  \num{+-0.37} &   7.56  \num{+-0.25} &   23.67  \num{+-0.19} &   5.47  \num{+-0.08} &   4.83  \num{+-0.11} &   5.01  \num{+-0.04} &   4.72  \num{+-0.03} &   3.96  \num{+-0.05} &   5.12  \num{+-0.07} &   20.67  \num{+-0.4} &   11.34  \num{+-0.2} & 11/15 \\

\bottomrule
Config. 3 \\
Source 1 &    8.58  \num{+-1.98} &   5.03  \num{+-0.43} &   4.76  \num{+-0.23} &   18.46  \num{+-6.72} &   21.18  \num{+-5.57} &   22.08  \num{+-0.34} &   28.93  \num{+-0.88} &   22.29  \num{+-0.78} &   7.09  \num{+-0.09} &   35.93  \num{+-3.73} &   6.33  \num{+-0.51} &   5  \num{+-0.14} &   5.16  \num{+-0.09} &   4.86  \num{+-0.15} &   4.45  \num{+-0.19} &   5.7  \num{+-0.42} &   24.81  \num{+-3} &   13.34  \num{+-1.46} & 5/15 \\
Source 2 &    9.34  \num{+-2.06} &   4.87  \num{+-0.25} &   4.89  \num{+-0.23} &   14.36  \num{+-1.48} &   16.98  \num{+-0.58} &   25.83  \num{+-0.61} &   31.97  \num{+-1.12} &   21.93  \num{+-0.71} &   7.86  \num{+-0.2} &   27.64  \num{+-0.53} &   9.03  \num{+-1.13} &   5.98  \num{+-0.27} &   6.15  \num{+-0.2} &   5.78  \num{+-0.15} &   5.21  \num{+-0.18} &   6.57  \num{+-0.52} &   23.12  \num{+-0.84} &   13.19  \num{+-0.65} & 5/15 \\
Source 3 &    5.25  \num{+-0.07} &   4.67  \num{+-0.05} &   4.61  \num{+-0.03} &   14.23  \num{+-0.39} &   16.23  \num{+-1.21} &   21.58  \num{+-0.27} &   28.64  \num{+-0.55} &   21.27  \num{+-0.57} &   7.45  \num{+-0.18} &   25.88  \num{+-0.24} &   6.02  \num{+-0.18} &   5.49  \num{+-0.08} &   5.5  \num{+-0.08} &   5.13  \num{+-0.1} &   4.79  \num{+-0.11} &   5.44  \num{+-0.1} &   21.3  \num{+-0.54} &   11.78  \num{+-0.27} & 8/15 \\
Source 4 &    \textbf{4.93}  \num{+-0.01} &   4.69  \num{+-0.04} &   4.6  \num{+-0.03} &   16.2  \num{+-0.56} &   14.9  \num{+-0.3} &   26.35  \num{+-1.6} &   31.09  \num{+-0.29} &   22.38  \num{+-0.28} &   7.64  \num{+-0.24} &   25.8  \num{+-0.27} &   6.15  \num{+-0.17} &   5.37  \num{+-0.12} &   5.36  \num{+-0.09} &   5.17  \num{+-0.1} &   4.58  \num{+-0.12} &   5.39  \num{+-0.1} &   22.79  \num{+-0.55} &   12.35  \num{+-0.28} & 7/15 \\
Source 5 &    5.01  \num{+-0.02} &   4.64  \num{+-0.03} &   \textbf{4.54}  \num{+-0.01} &   16.42  \num{+-0.39} &   20.3  \num{+-3.11} &   24.19  \num{+-1.82} &   30.78  \num{+-0.5} &   23.41  \num{+-0.39} &   8.58  \num{+-0.57} &   23.66  \num{+-0.15} &   6.24  \num{+-0.29} &   5.51  \num{+-0.23} &   5.45  \num{+-0.2} &   5.25  \num{+-0.18} &   4.67  \num{+-0.26} &   5.54  \num{+-0.2} &   23.13  \num{+-1.06} &   12.58  \num{+-0.54} & 8/15 \\
Source 6 &    5.34  \num{+-0.09} &   4.68  \num{+-0.04} &   4.62  \num{+-0.03} &   13.21  \num{+-0.82} &   15.1  \num{+-0.49} &   21.44  \num{+-0.09} &   28.72  \num{+-0.36} &   20.83  \num{+-0.33} &   7.22  \num{+-0.22} &   25.37  \num{+-0.31} &   5.72  \num{+-0.13} &   5.02  \num{+-0.16} &   5.17  \num{+-0.08} &   5  \num{+-0.11} &   4.48  \num{+-0.13} &   5.25  \num{+-0.11} &   20.78  \num{+-0.4} &   11.46  \num{+-0.23} & 8/15 \\
Source 7 &    5.02  \num{+-0.03} &   4.86  \num{+-0.07} &   4.6  \num{+-0.03} &   17.12  \num{+-0.59} &   14.15  \num{+-0.58} &   23.95  \num{+-0.26} &   33.66  \num{+-0.48} &   21.84  \num{+-0.11} &   7.3  \num{+-0.14} &   24.86  \num{+-0.17} &   5.89  \num{+-0.15} &   5.22  \num{+-0.12} &   5.33  \num{+-0.1} &   5.11  \num{+-0.09} &   4.51  \num{+-0.13} &   5.31  \num{+-0.1} &   22.6  \num{+-0.37} &   12.23  \num{+-0.2} & 7/15 \\
Source 8 &    4.97  \num{+-0.02} &   4.81  \num{+-0.07} &   4.6  \num{+-0.03} &   16.67  \num{+-0.39} &   16.77  \num{+-0.28} &   25.52  \num{+-0.34} &   35.47  \num{+-0.56} &   22.76  \num{+-0.12} &   11.47  \num{+-0.28} &   30.04  \num{+-0.3} &   9.46  \num{+-0.27} &   8.05  \num{+-0.25} &   6.78  \num{+-0.2} &   6.17  \num{+-0.18} &   5.39  \num{+-0.18} &   6.86  \num{+-0.16} &   24.54  \num{+-0.33} &   13.93  \num{+-0.23} & 6/15 \\
Source 9 &    5.06  \num{+-0.05} &   4.77  \num{+-0.06} &   4.6  \num{+-0.03} &   17.04  \num{+-0.62} &   16.46  \num{+-0.62} &   26.34  \num{+-2.15} &   29.2  \num{+-0.59} &   20.97  \num{+-0.13} &   8.23  \num{+-0.54} &   26.05  \num{+-0.38} &   6.01  \num{+-0.17} &   5.74  \num{+-0.25} &   5.5  \num{+-0.15} &   5.32  \num{+-0.2} &   4.64  \num{+-0.18} &   5.54  \num{+-0.18} &   22.68  \num{+-0.75} &   12.4  \num{+-0.41} & 8/15 \\
Source 10 &    5.14  \num{+-0.04} &   4.81  \num{+-0.08} &   4.65  \num{+-0.03} &   16.32  \num{+-0.78} &   16.39  \num{+-0.36} &   23.95  \num{+-0.35} &   33.63  \num{+-0.57} &   22.25  \num{+-0.19} &   7.79  \num{+-0.28} &   24.93  \num{+-0.3} &   6.35  \num{+-0.19} &   5.51  \num{+-0.18} &   5.37  \num{+-0.15} &   5.22  \num{+-0.16} &   4.6  \num{+-0.15} &   5.5  \num{+-0.14} &   22.91  \num{+-0.43} &   12.46  \num{+-0.25} & 7/15 \\
Source 11 &    5.32  \num{+-0.13} &   4.76  \num{+-0.06} &   4.63  \num{+-0.03} &   14.81  \num{+-0.33} &   15.24  \num{+-0.38} &   22.93  \num{+-0.34} &   29.1  \num{+-0.34} &   21.84  \num{+-0.68} &   7.75  \num{+-0.32} &   24.99  \num{+-0.39} &   6.06  \num{+-0.34} &   5.3  \num{+-0.18} &   5.26  \num{+-0.14} &   5.14  \num{+-0.16} &   4.48  \num{+-0.14} &   5.41  \num{+-0.17} &   21.48  \num{+-0.41} &   11.84  \num{+-0.27} & 7/15 \\
Source 12 &    5.1  \num{+-0.04} &   4.74  \num{+-0.05} &   4.62  \num{+-0.03} &   16.5  \num{+-0.72} &   15.48  \num{+-0.68} &   21.96  \num{+-0.16} &   30.01  \num{+-0.37} &   20.6  \num{+-0.23} &   7.27  \num{+-0.21} &   24.29  \num{+-0.37} &   5.95  \num{+-0.23} &   5.32  \num{+-0.13} &   5.28  \num{+-0.12} &   5.04  \num{+-0.1} &   4.5  \num{+-0.13} &   5.31  \num{+-0.11} &   21.47  \num{+-0.42} &   11.78  \num{+-0.24} & 9/15 \\
Source 13 &    5.28  \num{+-0.09} &   4.77  \num{+-0.06} &   4.62  \num{+-0.03} &   15.56  \num{+-0.43} &   15.5  \num{+-0.66} &   22.23  \num{+-0.46} &   30.06  \num{+-0.68} &   \textbf{20.07}  \num{+-0.09} &   7.54  \num{+-0.15} &   25  \num{+-0.4} &   5.86  \num{+-0.22} &   5.2  \num{+-0.16} &   5.33  \num{+-0.12} &   5.11  \num{+-0.14} &   4.45  \num{+-0.19} &   5.35  \num{+-0.13} &   21.4  \num{+-0.45} &   11.77  \num{+-0.26} & 8/15 \\
Source 14 &    5.14  \num{+-0.05} &   4.79  \num{+-0.06} &   4.65  \num{+-0.04} &   15.67  \num{+-0.39} &   15.56  \num{+-1.34} &   22.44  \num{+-0.37} &   31.43  \num{+-0.55} &   21  \num{+-0.09} &   10.94  \num{+-0.56} &   25.18  \num{+-0.39} &   7.85  \num{+-0.31} &   6.01  \num{+-0.21} &   6.23  \num{+-0.2} &   5.88  \num{+-0.14} &   5.04  \num{+-0.22} &   6.28  \num{+-0.2} &   21.88  \num{+-0.52} &   12.52  \num{+-0.33} & 7/15 \\



\end{tabular}

==> table_results_ens_all.tex <==
\begin{tabular}
  {@{} 
    lccccccccccccccc|cccc
  @{}}
  \toprule
      & \multicolumn{15}{c}{Validation weeks} &
      \multicolumn{4}{c}{Average results} & \\
    &  \multicolumn{1}{c} {W3} & {W4} & {W5} & \underline{{W6}}& \underline{{W7}}& \underline{{W8}}& \underline{{W9}}& \underline{{W10}}& {W11}& \underline{{W12}}& {W13}& {W14}& {W15}& {W16}& {W17}& {Weeks w/o promo}& \underline{{Weeks w/ promo}}& {Weeks total} & {Improvement}\\
  \midrule
w/o Transfer &  6.26 \num{+-1.06} &  5.16 \num{+-0.58} &  4.7 \num{+-0.2} &  29.12 \num{+-12.06} &  27.67 \num{+-8.5} &  \textbf{20.92} \num{+-0.44} &  28.04 \num{+-0.46} &  21.65 \num{+-1.19} &  10.8 \num{+-4.13} &  24.69 \num{+-1.69} &  5.53 \num{+-0.3} &  4.87 \num{+-0.27} &  4.98 \num{+-0.11} &  4.68 \num{+-0.1} &  3.95 \num{+-0.18} &  5.66 \num{+-0.77} &  25.35 \num{+-4.06} &  13.53 \num{+-2.08} &   \\
Naive & 5.80 & 5.28 & 5.05 & 14.71 & 16.90 & 23.03 & 31.20 & 21.79 & 9.79 & 26.72 & 7.65 & 6.97 & 6.37 & 6.41 & 5.65 & 6.55 & 22.39 & 12.89 & \\
 \bottomrule
All &  5.19 \num{+-0.05} &  4.65 \num{+-0.01} &  \textbf{4.55} \num{+-0.01} &  14.08 \num{+-0.49} &  \textbf{13.96} \num{+-0.13} &  21.05 \num{+-0.08} &  27.83 \num{+-0.14} &  20.62 \num{+-0.15} &  7.03 \num{+-0.05} &  24.02 \num{+-0.18} &  5.57 \num{+-0.13} &  4.73 \num{+-0.03} & \textbf{4.9} \num{+-0.01} &  4.63 \num{+-0.02} &  3.93 \num{+-0.02} &  5.02 \num{+-0.03} &  20.26 \num{+-0.2} &  11.12 \num{+-0.1} & \textbf{14/15} \\
Mean Sales High &   4.98 \num{+-0.02} &  4.67 \num{+-0.02} &  \textbf{4.55} \num{+-0.01} &  14.72 \num{+-0.4} &  14.07 \num{+-0.25} &  21.23 \num{+-0.13} &  28.09 \num{+-0.2} &  20.44 \num{+-0.2} &  7.18 \num{+-0.08} &  23.5 \num{+-0.17} &  5.45 \num{+-0.09} &  4.74 \num{+-0.05} &  4.91 \num{+-0.01} &  \textbf{4.62}  \num{+-0.02} &  3.93 \num{+-0.03} &  5 \num{+-0.12} &  20.34 \num{+-0.53} &  11.45 \num{+-0.28} & 13/15 \\
Mean Sales Medium &   5.15 \num{+-0.03} &  4.74 \num{+-0.03} &  4.59 \num{+-0.01} &  14.03 \num{+-0.17} &  14.36 \num{+-0.21} &  21.33 \num{+-0.17} &  28.03 \num{+-0.25} &  20.54 \num{+-0.16} &  7.2 \num{+-0.09} &  23.49 \num{+-0.17} &  5.4 \num{+-0.05} &  4.75 \num{+-0.04} &  4.91 \num{+-0.01} &  4.65 \num{+-0.03} &  3.94 \num{+-0.03} &  5.04 \num{+-0.04} &  20.3 \num{+-0.22} &  11.14 \num{+-0.11} & \textbf{14/15} \\
Mean Sales Low &   6.11 \num{+-0.34} &  \textbf{4.59} \num{+-0.02} &  \textbf{4.55} \num{+-0.02} &  13.78 \num{+-1.67} &  14.24 \num{+-0.11} &  21 \num{+-0.1} &  \textbf{27.73} \num{+-0.17} &  21.93 \num{+-0.66} &  \textbf{6.85} \num{+-0.04} &  26.29 \num{+-0.44} &  6.37 \num{+-0.53} &  4.72 \num{+-0.04} &  4.92 \num{+-0.03} &  4.63 \num{+-0.03} &  3.96 \num{+-0.06} &  5.19 \num{+-0.03} &  20.83 \num{+-0.19} &  11.14 \num{+-0.1} & 10/15 \\
Price High &  7.03 \num{+-0.64} &  4.65 \num{+-0.04} &  4.59 \num{+-0.03} &  15.1 \num{+-2.87} &  14.92 \num{+-0.3} &  21.29 \num{+-0.18} &  27.77 \num{+-0.2} &  23.47 \num{+-1.12} &  6.97 \num{+-0.05} &  26.39 \num{+-0.4} &  7.12 \num{+-0.87} &  4.77 \num{+-0.03} &  4.95 \num{+-0.03} &  4.66 \num{+-0.05} &  3.99 \num{+-0.05} &  5.41 \num{+-0.2} &  21.49 \num{+-0.84} &  11.84 \num{+-0.46} & 12/15  \\
Price Medium &   5.02 \num{+-0.03} &  4.64 \num{+-0.02} &  4.56 \num{+-0.01} &  \textbf{13.16} \num{+-0.37} &  14.14 \num{+-0.25} &  21.1 \num{+-0.14} &  27.8 \num{+-0.2} &  20.41 \num{+-0.19} &  7.1 \num{+-0.09} &  23.71 \num{+-0.18} &  \textbf{5.38} \num{+-0.07} &  \textbf{4.71} \num{+-0.04} & \textbf{4.9} \num{+-0.01} &  4.63 \num{+-0.02} &  3.92 \num{+-0.03} &  \textbf{4.98}  \num{+-0.04} &  \textbf{20.05}  \num{+-0.22} &  \textbf{11.01} \num{+-0.11} & \textbf{14/15} \\
Price Low &  5.04 \num{+-0.02} &  4.73 \num{+-0.02} &  4.57 \num{+-0.01} &  14.83 \num{+-0.2} &  14.17 \num{+-0.24} &  21.16 \num{+-0.12} &  28.21 \num{+-0.25} &  20.37 \num{+-0.18} &  7.07 \num{+-0.06} &  23.64 \num{+-0.23} &  5.4 \num{+-0.08} &  4.75 \num{+-0.05} & \textbf{4.9} \num{+-0.01} &  4.64 \num{+-0.02} &  3.93 \num{+-0.02} &  5 \num{+-0.03} &  20.4 \num{+-0.2} &  11.16 \num{+-0.1} & 10/15 \\
Promo High &   \textbf{4.95} \num{+-0.02} &  4.64 \num{+-0.02} &  4.56 \num{+-0.01} &  15.84 \num{+-0.25} &  14.97 \num{+-0.65} &  21.67 \num{+-0.39} &  28.89 \num{+-0.29} &  \textbf{20.32} \num{+-0.15} &  7.76 \num{+-0.2} &  \textbf{23.48} \num{+-0.39} &  5.55 \num{+-0.14} &  4.77 \num{+-0.08} &  4.94 \num{+-0.02} &  \textbf{4.62}  \num{+-0.02} &  3.92 \num{+-0.04} &  5.08 \num{+-0.22} &  20.86 \num{+-0.93} &  11.39 \num{+-0.5} & 12/15 \\
Promo Medium &   5.09 \num{+-0.06} &  4.7 \num{+-0.03} &  4.57 \num{+-0.01} &  13.91 \num{+-0.72} &  14.33 \num{+-0.64} &  21.22 \num{+-0.24} &  27.91 \num{+-0.25} &  20.53 \num{+-0.17} &  7.14 \num{+-0.27} &  23.52 \num{+-0.1} &  5.4 \num{+-0.04} &  4.74 \num{+-0.04} & \textbf{4.9} \num{+-0.01} &  4.64 \num{+-0.02} &  3.94 \num{+-0.02} &  5.01 \num{+-0.06} &  20.24 \num{+-0.35} &  11.10 \num{+-0.18} & \textbf{14/15} \\
Promo Low &   6.47 \num{+-0.7} &  4.62 \num{+-0.04} &  4.57 \num{+-0.03} &  14.79 \num{+-2.52} &  15.05 \num{+-0.48} &  21.03 \num{+-0.14} &  27.8 \num{+-0.21} &  22.59 \num{+-1.02} &  6.89 \num{+-0.05} &  27.14 \num{+-1.22} &  6.81 \num{+-0.96} &  4.72 \num{+-0.04} &  4.93 \num{+-0.04} &  4.64 \num{+-0.03} &  3.97 \num{+-0.07} &  5.29 \num{+-0.06} &  21.4 \num{+-0.35} &  11.73 \num{+-0.18} & 9/15 \\




\end{tabular}
